Mechanism Design for Perturbation Stable Combinatorial Auctions

Motivated by recent research on combinatorial markets with endowed valuations by (Babaioff et al., EC 2018) and (Ezra et al., EC 2020), we introduce a notion of perturbation stability in Combinatorial Auctions (CAs) and study the extend to which stability helps in social welfare maximization and mechanism design. A CA is $\gamma\textit{-stable}$ if the optimal solution is resilient to inflation, by a factor of $\gamma \geq 1$, of any bidder's valuation for any single item. On the positive side, we show how to compute efficiently an optimal allocation for 2-stable subadditive valuations and that a Walrasian equilibrium exists for 2-stable submodular valuations. Moreover, we show that a Parallel 2nd Price Auction (P2A) followed by a demand query for each bidder is truthful for general subadditive valuations and results in the optimal allocation for 2-stable submodular valuations. To highlight the challenges behind optimization and mechanism design for stable CAs, we show that a Walrasian equilibrium may not exist for $\gamma$-stable XOS valuations for any $\gamma$, that a polynomial-time approximation scheme does not exist for $(2-\epsilon)$-stable submodular valuations, and that any DSIC mechanism that computes the optimal allocation for stable CAs and does not use demand queries must use exponentially many value queries. We conclude with analyzing the Price of Anarchy of P2A and Parallel 1st Price Auctions (P1A) for CAs with stable submodular and XOS valuations. Our results indicate that the quality of equilibria of simple non-truthful auctions improves only for $\gamma$-stable instances with $\gamma \geq 3$.

==> 3-stability.tex <==
\section{Properties of Perturbation Stable Valuations}\label{sec:stability}


% \subsection{Definition of Perturbation Stability}

% In order to define perturbation stability for combinatorial auctions, first we need to define how to perturb an instance of an auction.

% \begin{definition}[Perturbation of Valuations]
%     For any $\g\geq 1$, a \textit{$\g$-perturbation} of a vector of valuations $\vv$ is another vector of valuations $\vv'$, where for one bidder $i\in N$, one item $j\in M$ and some $\sigma\in [1,\g]$:
%     \begin{itemize}
%         \item $\vv'_{-i}=\vv_{-i}$
%         \item $v_i'(S) = v_i(S) + (\sigma-1)\cdot v_i(S\cap\{j\})$, for every $S\sub M$
%     \end{itemize}
% \end{definition}

% Simply put, the above perturbation keeps every valuation the same, except for one, which is endowed for one item.

% Having defined how to perturb some valuations, we are ready to define what perturbation stable valuations are.

% \begin{definition}[Perturbation-Stability]
%     For any $\g\geq 1$, an vector of valuations is called \textit{$\g$-perturbation stable}, or simply \textit{$\g$-stable}, if the optimal allocation is unique, and remains unique under any $\g$-perturbation.
% \end{definition}

% To add some intuition to the definition above, it simply states that the optimal allocation is strong enough, so that it remains optimal even if any single item is endowed for any single bidder, by at most $\g$. Let us present an example to make the definition even clearer.

% \begin{example} \label{AliceBobEx}
%     Let Alice and Bob be our 2 bidders, in an auction of 2 items $a$ and $b$. Alice and Bob have unit-demand valuations. Alice values item $a$ for $2$ and item $b$ for $1$. Bob is symmetrical, meaning he values $b$ for $2$ and $a$ for $1$. Clearly the optimal allocation is to allocate $a$ to Alice and $b$ to Bob, i.e. $O_A=\{a\}, O_B=\{b\}$. Let us calculate how stable this auction is.

%     First we notice that the optimal allocation is unique, which means that the auction is at least $1$-stable. In order to check what is the maximum value of $\g$, we need to find how much we need to endow some item for some bidder, in order for the allocation $(O_A, O_B)$ to be suboptimal. We easily notice that if we endow either Alice's value for item $a$, or Bob's value for item $b$ the optimal allocation will only get stronger. Since the bidders are symmetrical we only need to check what happens when we endow Alice's value for $b$.

%     If we endow by $\g$, her new values are $v_A'(b) = \g$ and $v_A'(ab) = \g+1$. Now the optimal allocation still has a social welfare of $4$ and any other allocation that could become optimal (giving $ab$ to Alice or $b$ to Alice and $a$ to Bob) has welfare equal to $\g + 1$. Thus in order for the optimal allocation to remain uniquely optimal it must hold that $4>\g+1$. This concludes that the auction is $(3-\e)$-stable or simply $\g$-stable, where $\g<3$. 
% \end{example}


In this section we explore some basic properties that derive from definition \ref{def:stability}. First we will see a basic, but fundamental property of stable valuations.

\begin{lemma}[Property of Stable Valuations] \label{LemmaGen}
    Let $\vv$ be $\g$-stable valuations. Then for every bidder $i$, every item in $i$'s optimal bundle $j\in O_i$ and any other bidder $k\neq i$
    \begin{equation*}
        v_i(O_i) - v_i(O_i-j) > (\g-1)\cdot v_k(j)
    \end{equation*}
\end{lemma}

\begin{proof}
    Fix an arbitrary bidder $i$, an item $j\in O_i$ and another bidder $k$, whose optimal set is $O_k$. Since the valuations are $\g$-stable, the optimal allocation will stay unique if we endow $k$'s value for item $j$ by $\g$, changing $k$'s valuation to $v_k'(S) = v_k(S) + (\g-1)\cd v_k(j\cap S)$. In the perturbed auction we compare the optimal allocation with the allocation which is the same as the optimal, but $j$ goes to bidder $k$ instead of $i$:
    \begin{equation*}
        \sum_{l\neq i,k}v_l(O_l) + v_i(O_i) + v_k'(O_k) > \sum_{l\neq i,k}v_l(O_l) + v_i(O_i-j) + v_k'(O_k\cup j)
    \end{equation*}

    Combining that $v_k(O_k\cup j) - v_k(O_k) \geq 0$ ($v_k$ is non-decreasing) and the above inequality yields the lemma.
\end{proof}

Now we see the application of this lemma to specific classes of valuations.

\begin{corollary}[Corollary of Stable Valuations] \label{cor:basic}
    Let $\vv$ be a $\g$-stable. Then for every bidder $i$, every item in $i$'s optimal bundle $j\in O_i$ and any bidder $k\neq i$
    \begin{itemize}
        \item If $\vv$ are subadditive, then $v_i(j) > (\g-1)\cd v_k(j)$.
        \item If $\vv$ are XOS and $q_i(\cdot)$ supports $i$'s optimal bundle, then $q_i(j) > (\g-1)\cdot v_k(j)$.
        \item If $\vv$ are submodular, then $v_i(S) - v_i(S-j) > (\g-1)\cdot v_k(j)$.
    \end{itemize}
\end{corollary}

% Because all of these properties come immediately from the properties of each valuation class the proof is emitted.
\checknote{Should we put the proof in the appendix?}. 

% With these corollaries we are going to prove the majority of the theorems that will follow in the rest of the paper. Given that our valuations are stable first we are going to show that that finding that optimal allocation is easier, even in subadditive valuations. Then we are going to improve known results for auctions with selfish bidders and finally we are going to improve the bounds associated with the Price of Anarchy in simple auctions.
